ChatGLM: A Family of Large Language Models from GLM-130B to GLM-4 All Tools

We introduce ChatGLM, an evolving family of large language models that we have been developing over time. This report primarily focuses on the GLM-4 language series, which includes GLM-4, GLM-4-Air, and GLM-4-9B. They represent our most capable models that are trained with all the insights and lessons gained from the preceding three generations of ChatGLM. To date, the GLM-4 models are pre-trained on ten trillions of tokens mostly in Chinese and English, along with a small set of corpus from 24 languages, and aligned primarily for Chinese and English usage. The high-quality alignment is achieved via a multi-stage post-training process, which involves supervised fine-tuning and learning from human feedback. Evaluations show that GLM-4 1) closely rivals or outperforms GPT-4 in terms of general metrics such as MMLU, GSM8K, MATH, BBH, GPQA, and HumanEval, 2) gets close to GPT-4-Turbo in instruction following as measured by IFEval, 3) matches GPT-4 Turbo (128K) and Claude 3 for long context tasks, and 4) outperforms GPT-4 in Chinese alignments as measured by AlignBench. The GLM-4 All Tools model is further aligned to understand user intent and autonomously decide when and which tool(s) touse -- including web browser, Python interpreter, text-to-image model, and user-defined functions -- to effectively complete complex tasks. In practical applications, it matches and even surpasses GPT-4 All Tools in tasks like accessing online information via web browsing and solving math problems using Python interpreter. Over the course, we have open-sourced a series of models, including ChatGLM-6B (three generations), GLM-4-9B (128K, 1M), GLM-4V-9B, WebGLM, and CodeGeeX, attracting over 10 million downloads on Hugging face in the year 2023 alone. The open models can be accessed through https://github.com/THUDM and https://huggingface.co/THUDM.

==> 9_backup.tex <==
\section{\model: Architecture, Data, and Training}






\model is a bilingual LLM that masters instructions, queries, and dialogues in both Chinese and English.
To allow its capability, considerate efforts are paid on studying the model architectures, data distributions, and alignment techniques.




\subsection{Architecture}
Following its predecessors~\cite{du2022glm,zeng2022glm}, \model adopts the General Language Model (GLM) architecture~\cite{du2022glm}, allowing a flexible mixture of pre-training objectives and strong performances.
In the development of \model, we identify two architectural choices that are essenstial for its training and inference efficiency, including Rotary Positional Encoding~\cite{su2021roformer} and Multi-query Attention~\cite{shazeer2019fast}.

\vpara{Rotary Positional Encoding (RoPE).}
Besides RoPE' recently demonstrated capability to interpolate for strong performance in long context inference~\cite{chen2023extending}, it is also worth noticing that compared to other relative PE options (e.g., ALiBi~\cite{press2022train}), RoPE is likely a must for FlashAttention (Cf. Section~\ref{sec:inference}), which is a recomputation technique to dramatically boost LLMs' inference-time efficiency.
Therefore, in \model we continue to adopt RoPE as we previously also did in GLM-130B~\cite{zeng2022glm}.

\vpara{Multi-query Attention.}
Another important architectural optimization in \model is the multi-query attention~\cite{shazeer2019fast} that also being adopted by PaLM~\cite{chowdhery2022palm}, which only keep one of the $n_{\text{head}}$ key and value attention heads.
In both its original experiments and our practices, we find it to drastically improve decoding speed and run-time memory with a tolerable loss in accuracy.

\todo{Model hyperparameters}

\subsection{Pre-training}
To endow \model strong bilingual language abilities, we carefully collect, filter, and experiment on a large amounts of Chinese and English corpora.
\model is finally pre-trained over 1.4T bilingual tokens over texts from various sources.

\vpara{Data.}
A dominant challenge in pre-training is to acquire high-quality and diverse pre-training corpora.
To achieve the mission, we develop a systematic data preparation pipeline as follow:

\begin{itemize}[leftmargin=1.5em,itemsep=0pt,parsep=0.2em,topsep=0.0em,partopsep=0.0em]
\item \textbf{Collecting}: The majority of our pre-training corpora comes from publicly available webpage contents. Other sources include some existing book datasets and code from public GitHub repos.
\item \textbf{Cleaning}: While web corpora are diverse enough, they vary in qualities. First, we leverage rule-based strategies to filter webpages from low-quality urls and content-sensitive keywords. Similar to literature~\cite{gao2020pile}, we then employ a strong document classifier to find high-quality pages.
\item \textbf{Deduplication}: Web contents are often duplicated. We adopt the standard MinHash~\cite{broder1997resemblance} algorithm to deduplicate web contents for higher quality data composition.
\end{itemize}

After carefully processing, we finally create \todo{} tokens of bilingual pre-training corpora with roughly equal proportion of Chinese and English texts.

\vpara{Training.}
To efficiently pre-train LLMs is difficult.
In the pre-training of \model, we set up a framework enabled with multiple parallel strategies to scale up training efficiency, including data parallelism~\cite{dean2012large}, tensor parallelism~\cite{shoeybi2019megatron}, pipeline parallelism~\cite{huang2019gpipe}, and sequence parallelism~\cite{korthikanti2023reducing}.
\model series all adopt BF16 floating-point precision, which reduces training instabilities. 

\vpara{32k Long Context in Pre-training.}
Additionally, another core improvement for \model is the extension of context length from 2k to 32k in pre-training.
In the past~\cite{}, people have assumed that standard attention's quadratic complexity would do harm to transformer's training on long contexts.
Nevertheless,  researchers have recently come to realize that when context length is not significantly larger than hidden size, the disadvantage is trivial.
A potentially efficiency problem lies in inference, but could now be properly tackled  by FlashAttention~\cite{dao2022flashattention} when context length is smaller than 100k.

\subsection{Alignment Training}
After sufficient pre-training, \model has been equipped rather strong language skills.
However, it is still a base LLM that poorly understand human intentions, follow complicated instructions, and communicate in multi-turn dialogues.
As a result, the alignment training~\cite{ouyang2022training} is critical for \model's practical use and deployment for applications.
Generally speaking, \model takes the following steps to align itself to human preference:

\begin{itemize}[leftmargin=1.5em,itemsep=0pt,parsep=0.2em,topsep=0.0em,partopsep=0.0em]
\item \textbf{Supervised Fine-tuning (SFT)}: We collect initial queries by our existing web demonstrations (after data desensitization) and annotators' creation, including both single-round and multi-round ones. Annotators will then correctify and polish model generated answers to form the SFT corpus. In practice, we find authentic human prompts and interactions instead of template-based or model generated ones are vital to LLMs' quality when providing services to real users.
\item \textbf{Feedback Bootstrapping (FB)}: An important step to improve \model quality is to iteratively select out high-quality answers for training. We instruct annotators to score model responses from several dimensions, including safety, factuality, relevance, helpfulness, and human preferences. Only top-scored responses by annotators are added to the next iteration of training. This feedback bootstrapping period is conducted for dozens of iterations over a diverse range of topics.
\item \textbf{Reinforcement Learning From Human Feedback (RLHF)}: After SFT and FB, \model has been quite aligned to human intentions and preferences. However, we notice that \model still has flaws in specific tasks and situations, such as rejecting responses, safety issues, generating mixture of bilingual tokens, multi-turn coherence, and some typical tasks. Our experiments show that it is RLHF rather than SFT or FB can help to substantially mitigate these problems.
\end{itemize}

\vpara{Alignment Tax on Academic Datasets.}
While alignment is necessary for practical use, as is also noted in InstructGPT~\cite{ouyang2022training}, an alignment tax for chat-aligned \model is paid on academic datasets compared to its base version, despite using strategies like mixing pre-training corpora in alignment.

\subsection{Inference} \label{sec:inference}
Inference efficiency is a key for LLMs' practical deployment and applications.
As is reported, inference costs for serving GPT-4 to millions of users could be magnitudes larger than training it from scratch.
Thus, a major design focus of \model has been on improving inference performance.

\vpara{KV Cache.}
While bidirectional PrefixLM-style processing of context has been demonstrated to have strong performance~\cite{du2022glm,zeng2022glm}, in practice it has increased first-word responding latency.
To improve \model-6B's user experience in local single-thread deployment, we adopt KV Cache with causal mask in the official implementation for \model-6B's local inference.

\vpara{FlashAttention.}
Transformer's quadratic complexity has been a major obstacle in scaling LLMs' context lengths.
While previous efficient transformers' focus has been on reducing the attention computation FLOP,~\cite{dao2022flashattention} notices that an often neglected bottleneck lies in the IO.
Thus, FlashAttention drastically speeds up and saves GPU memory usage by employing attention recomputation to avoid memory access.
In \model, we also adopt FlashAttention for better speed and space usage .

